Optomechanical entanglement at room temperature: a simulation study with realistic conditions

Quantum entanglement is the key to many applications like quantum key distribution, quantum teleportation, and quantum sensing. However, reliably generating quantum entanglement in macroscopic systems has proved to be a challenge. Here, we present a detailed analysis of ponderomotive entanglement generation which utilizes optomechanical interactions to create quantum correlations. We numerically calculate an entanglement measure -- the logarithmic negativity -- for the quantitative assessment of the entanglement. Experimental limitations, including thermal noise and optical loss, from measurements of an existing experiment were included in the calculation, which is intractable to solve analytically. This work will play an important role in the development of ponderomotive entanglement devices.

==> sum250.tex <==
Many if not most quantum technologies require a source of entangled particle or photons. A future society that efficiently uses quantum technologies would rely on entanglement, likely entangled photons, as society today relies on electricity. We computationally explored a novel method to entangle beams of photons. This method is commonly referred to as optomechanical entanglement generation. 

Optomechanical entanglement traditionally (or usually) involves an optical cavity whose overall length is determined by the incident light’s force on a movable mirror. An optical cavity is device that temporarily traps incoming light and through resonance amplifies it. Here, the cavity is used to amplify the quantum radiation pressure noise incident on the movable mirror. 

Whereas radiation pressure is the force electromagnetic radiation exerts on a material surface, quantum radiation pressure is the radiation pressure from the fundamental (think Heisenberg’s uncertainty principle) uncertainty in the amplitude of the electromagnetic wave. This effect is a significant source of noise for many measurements and experiments. However, in optomechanics that noise source can be manipulated into an entanglement source. Our work explores this application, within a reasonable parameter space, computationally with realistic noise models. Contrary to previous publications, we found that entanglement production method generates entanglement at room temperature. Furthermore, we found that reducing loss and temperature increase the output entanglement from the system.  We also consider the higher order modes of our oscillator; at these frequencies the system produces no entanglement. 

This study helps focus our laboratory approach, and enables more expansive computational research in optomechanical entanglement and quantum cavity optomechanics. 

(256)



